Benchmarking Popular Classification Models' Robustness to Random and Targeted Corruptions

Text classification models, especially neural networks based models, have reached very high accuracy on many popular benchmark datasets. Yet, such models when deployed in real world applications, tend to perform badly. The primary reason is that these models are not tested against sufficient real world natural data. Based on the application users, the vocabulary and the style of the model's input may greatly vary. This emphasizes the need for a model agnostic test dataset, which consists of various corruptions that are natural to appear in the wild. Models trained and tested on such benchmark datasets, will be more robust against real world data. However, such data sets are not easily available. In this work, we address this problem, by extending the benchmark datasets along naturally occurring corruptions such as Spelling Errors, Text Noise and Synonyms and making them publicly available. Through extensive experiments, we compare random and targeted corruption strategies using Local Interpretable Model-Agnostic Explanations(LIME). We report the vulnerabilities in two popular text classification models along these corruptions and also find that targeted corruptions can expose vulnerabilities of a model better than random choices in most cases.

==> 1_intro_shreya.tex <==
\section{Introduction}


\begin{figure*}
\centering
\includegraphics[width=\textwidth]{nlds.png}
\caption{An example of the Neural Layer Definition Standard (NLDS) for the popular LSTM layer, along with their corresponding Caffe Prototxt and Keras python code.}
\label{fig:sys_arch_nlds}
\end{figure*}

Over the past decade, deep learning based systems have shown tremendous success for various tasks like speech recognition\cite{}, computer vision \cite{} and is widely adopted in safety-critical systems like \cite{}. While designing such a system we desire that the system performs well on a realm of different domains comprising of varied and realistic data. 

Humans have the ability to map the data comprising of various variations, corruptions and perturbation and hence can perform better than any existing systems. Humans are not muddled by variation like blur, rotation etc. in the input image.  Additionally, they are successfully able to comprehend text which is expressed in a varied way. The variations may range from text length, use of emoticons, formal vs informal expression, use of abbreviations, vocabulary, and grammatical style like voice, tense etc.   

Majority of systems the performance is based on the training data at hand. Typically, the training data consists of samples from a limited number of distributions, resulting in unsatisfactory performance when the model has to process data from the unseen distribution.  The vast scope of training data and humans ability to recognize various forms of representations make the human performance at par with models and vulnerable, sensitive to slight variations. 

\todo{Connect it to the previous para / re-arrange}
Now-days, deep learning based text classification plays an a 
important role is in processing plethora of information. For instance, recommendation system heavily rely on the sentiment analysis  on user reviews and comments~\cite{MEDHAT20141093}.
On the other hand, text classification is extremely important for enhancing the safety of online discussion environments, e.g., automatically detect online toxic content ~\cite{toxicdata} like irony, sarcasm etc. 
\todo{Add some real examples or stories.}

Given this increase in use of text classification models it has become extremely important to understand systems behaviour for uncommon inputs. Currently, majority of models are evaluated based on their performance on limited data and hence there are no guarantees of its performance on unseen and rare inputs. As shown by event where Google self-driven car crashed into a bus because it expected the bus to yield under a set of rare conditions but bus did not \cite{googleacc}.  Such incidents give rise to need of good model performance on good quality test data. Using an inadequate test data-set, models that have achieved high test accuracy may still lack generality and robustness.

In this work, we propose a framework, that can effectively  test the sensitivity of various deep learning models by bench-marking them against generated test samples considering various forms of corruptions. Our contributions can be summarized as:
\begin{enumerate}
    \item A framework to generate test suite for testing sensitivity and vulnerability of adversarial models. 
    \item The framework proposed is not aware about the model internal to generate a test suite(Black-Box).
    \item The framework generates a high quality test suite comprising of corruptions by using various augmentation strategies like synonym replacement, typos, noise addition and paraphrase. 
    \item The framework proposes two strategy for corruption targeted and random.  \todo{Utkarsh please check this} 
    \item Our empirical analysis state that these models are are sensitive to small amounts of natural variations introduced in the test set. 
\end{enumerate}


\begin{comment}
Outline: 
human ability to understand text is much several leagues ahead of existing learning systems. 

variation in human expression 
1. length 
2. emoticons 
3. formal & informal 
4. abbreviations 
5. voice 
6. use of vocab 

model needs to cater to dimensions 
1. typos: 
2. noise 
(Table / figure )
some examples etc .. some citations 
"diagram of an examples" 

testing papers:
why to test text models ?? 
what is sensitivity of  text models 
difference with adversary 

Our contribution 
 
Related work: 
testing work --- emphasis most are in images 
challenges with text when compared to image??
work in text ?? -- no work yet 
related work to introduce errors and  cite augmentation work and clearly state the difference 


Approach 
Block diagram -- 
Experiments 
\end{comment}

% \label{intro}
% Data has proven to be one of the primary factors behind the success of Artifical Intelligent (AI) applications. Most of the AI applications are developed using deep learning models which have proven to be very successful in automatically extracting complex and intricate features from data. As the name suggests, deep learning models are complicated architectures consisting of several layers of transformation and hyper-parameter options (in the order of millions). There has been a paramount of research performed in automating the task of finding best models and architectures for a given dataset and task ~\cite{zoph2017neural} ~\cite{pham2018efficient}. Researchers have characterized deep learning models ~\cite{deng2017peephole}, analyzed the shortcomings of a model for a given task, and dynamically modified the model to achieve better performance~\cite{cai2018efficient}. Further in the search for the best model for a given dataset task, the current research process tends to overfit the deep learning architecture to only achieve best results in that benchmark dataset with a loss of cross-dataset generalization. 

% However, it is understood that a model is only as good as the input training data. Thus, if the training data is insufficient in terms of volume or variety, then even the performance of a complicated deep learning model will be poor. In the literature, there has been a relatively lesser focus in characterizing the input data, as compared to characterizing the deep learning model. In this research, our primary aim is to automatically characterize and improve the quality of a given dataset in a trainless manner.

% Data augmentation is a common technique adopted for improving the data quality. To be able to learn a deep learning model from limited training data, there are broadly four different types of data augmentation strategies that exist:
% \begin{enumerate}
%     \item \textbf{Unlabeled data from same modality:} To be able to learn more robust features often unlabeled images from the same task or the same modality is augmented to the labeled dataset.
%     \item \textbf{Labeled data from related domain/tasks:} The limited labeled data from the target domain is augmented with some labeled data of a similar task from the source domain. The deep learning model is originally trained on the source domain labeled dataset and further adapted to the target data.
%     \item \textbf{Synthetic data generation:} By learning the distribution of given data, a generative model could be used to sample more data from the fitted distribution. Generative Adversarial Network (GAN) based data generation has gained some recent attention in the literature.
%     \item \textbf{Augmentation by transforming existing data:} Specific transformation functions such as affine transformation of images, variations of words could be performed to augment additional labeled data for training. The domain expertise and the prior dataset knowledge could be leveraged to choose the transformation functions.
%  \end{enumerate}

% As a motivating example, consider the typical model and data lifecyle in addressing CIFAR-10, which is a standard benchmark image dataset for object classification. To address this problem using some state-of-art deep learning models, the first step in practice would be to choose an ideal model architecture. The chosen architecture is trained using the benchmark train dataset to obtain the model's initial performance. To boost the performance of this model, as a thumb rule, data augmentation is performed in practice. Either certain specific augmentation strategies are adopted (which required human expertise) or certain random augmentation strategies such as flip and rotate the image are performed (which does not include any dataset properties). The model is trained using the augmented train dataset. Based on the obtained performance, further augmentation is performed and the cycle is repeated till expected performance is obtained. This whole iterative process is rather time-taking and random most often, resulting in decremental performance of the model.

%  Artificial intelligent (AI) application development, focuses on novelty and rigour in defining model architecture to enable a high quality AI application. There is considerably less focus in terms of analyzing the data that is available for learning/ training. If the data quality is not studied and improved upon, any amount of effort spent in searching for better model architectures and algorithms cannot guarantee high quality (say, accuracy) AI models. 

% For images, techniques have been proposed which can be used to  make image based model more robust. AutoAugment[1] from Google recommends improved augmentation policies for images by 1) Creating search space of data augmentation policies. 2) Evaluating the quality of a particular policy directly on the data-set of interest.
% However, this is model dependent and still computationally intensive and might not be always practical. With Subject Matter Experts (SME's) intervention all relevant transformations can be identified and applied that can enhance the quality of dataset substantially. Further irrelevant transformations can be ignored which will save the computation need. For example, applying flip or mirror on MNIST dataset's class having one digit doesn't make any sense and is a waste of computer resources.

% Despite good performance on benchmark data-sets,modern NLP techniques are nowhere near the skill of humans at language understanding or reasoning. Therefore, we propose few evaluation measures and provide insights on the data quality and strategies to augment data for better model performance.



==> 2_related_work_v1.tex <==
\section{Related Work}
\begin{comment}
Outline: 
testing work --- emphasis most are in images 
challenges with text when compared to image??
work in text ?? -- no work yet 
related work to introduce errors and  cite augmentation work and clearly state the difference 
\end{comment}

\textbf{Adversarial Examples}

Enormous attention has been given to robustness of the model towards adversarial examples and design of defence algorithms towards these adversaries.   Algorithms have been developed to search for minimal distortions to create an adversary by both being conscious (white-box) / unconscious(black-box) of the model specifics. Majority of work  \cite{ExplainingAH,adv_text,carlini1,Ebrahimi2017HotFlipWA}, have generated adversarial perturbations for image data. These work take into account imperceptible perturbations,\cite{rules_of_games} distinguished imperceptible perturbations with content preserving perturbations. The content-preserving perturbations encompass transformation that does not change the content significantly although the appearance may change slightly.  Recently the the focus in text adversarial generation \cite{Li2018TextBuggerGA,deeptext}\todo{add more citation fro text adversarial papers}.  
Our work does not aim to generate adversarial examples but generates test-cases from the data sets to asses the model thoroughly before deploying in safety-critical systems. 
\todo{add more details for clear distinction with adversarial work}

\textbf{Testing of deep learning systems}
\cite{testing1} propose a white-box framework for testing real-world DL-systems using measures like neuron coverage.  They successfully find many incorrect corner cases behaviours of the state of art model ImageNet \cite{} and on self-driving cars challenge data. Importance of a good quality test set is further emphasized by \cite{mutation_testing} using a white box mutation testing framework for image data. 
\cite{model_vulnerability}  asses the vulnerability of computer vision models to distributional shifts on an input image. 

\textbf{Challenges in text generation}
Natural Language data is difficult to process because of its symbolic, compositional and sparse, discrete in nature. These properties of text data prevent application of gradient-descent learning (and text GAN)  techniques and hence making it harder to generate realistic textual data. 

\textbf{Text augmentation Strategies}
\todo{Do we need it in the aspect of augmentation? Should it be augmentation or it should be more from text generation work}
%\textbf{Work in vision}
Data augmentation has shown tremendous success in its application in the field of computer vision.  Work like \cite{vision_da,Krizhevsky:2012:ICD:2999134.2999257, img_transforms} have shown geometric transformations  as useful technique to create new images by applying. Data augmentation in these areas can be easily performed by transformations like re-sizing, mirroring, random cropping, and colour shifting.  \cite{Perez2017TheEO} suggest the use of GANs to generate images of different styles and a new method to choose which additions are useful for the classifier.  Speech signal is manipulated using primitive operations like noise injection, spectrogram modification \cite{Ko2015AudioAF,2019arXiv190408779P} 


%\textbf{Challenges in text}


\cite{Mueller:2016:SRA:3016100.3016291} replaced random words in a sentence with their respective synonyms, to generate augmented data and train a Siamese recurrent network for sentence similarity task. \cite{wang-yang-2015-thats} used word embeddings of sentences to generate augmented data for the purpose of increasing data size and trained a multi-class classifier on tweet data. They found the nearest neighbour of a word vector by using cosine similarity and used that as a replacement for the original word. The word selection was done stochastically.

\cite{legal_text_analysis}  applied data augmentation techniques on legal data set. A class specific probability classifier was trained to identify a particular contract element type for each token in a sentence. They classified a token in a sentence based on the window of words/tokens surrounding them. They used word embeddings obtained by pretraining a word2vec model on unlabeled contract data.  Their work examined three data augmentation methods namely; interpolation, extrapolation and random noise. 

\cite{kobayashi-2018-contextual}
trained a bi-directional language model conditioned on class labels where it predicted the probability of a word based on the surrounding context of the words. The words with the best probability values were taken into consideration while generating the augmented sentences wherein the words in the sentences were replaced in a paradigmatic way

% \cite{risch-krestel-2018-aggress}  

\cite{Wei2019EDAED} suggest simple techniques based out of operation like synonym replacement, random insertion, random swap, and random deletion. They test these techniques on text classification models like CNN and RNN. 

==> 5_results.tex <==
\section{Discussion}

We first discuss the results of word deletion in tables 6 and 7. 

We now analyze the robustness of the two models separately for each dataset, in the context of the two corruption schemes. First, as expected, the accuracies of both models fall as the number of corrupted words in a document increases. This decrease in accuracy when compared to the original baselines is much greater on the SST2 dataset for both models. In general, the Bi-LSTM model seems to have much larger drops in accuracy than t
e FastText model (the blue dotted lines have higher slopes in all the plots than the red dashed lines). This is a very strong signal that the Bi-LSTM model used in our experiments is very vulnerable to corruptions. Additionally, both the models react strongly to introduction of spelling errors and text noise. We believe this is because these two methods could potentially change the semantics of a document, while replacing words is expected to preserve the original meaning. One minor anomaly we observe in the results, specifically for synonym-based corruption, is that the accuracy increases as we corrupt more words (for SST2 dataset, Bi-LSTM accuracy increases by $4.8\%$ and for IMDB dataset, FastText accuracy increases by $0.2\%$). We believe this increase is likely due to the replaced synonym was able to better convey the sentiment of the document.



==> noise.tex <==
\label{intro}
Noise in text data refers to the presence of any unnecessary characters that reduce the overall readability of text. The type and frequency of text noise depends greatly on the data source and the data collection mechanism. The overall effect is still reduction in readability and comprehension of text. Interestingly, in most cases, humans are still able to understand text with high noise levels. Noise can be present both at
Character  (CHRL) or Word level (WRDL). 

Table ~\ref{noise-table} list the techniques used for introducing noise to corrupt the text data. 

%\begin{enumerate}
    %\item \textbf{Random Characters} (CHRL): A random character is replaced by another random character. For example: problem --\textgreater  prxblem
   %\item \textbf{Punctuation} (CHRL): Unnecessary punctuation added in the text using ".!?,;:-{}()[]" punctuation marks. For example: problem --\textgreater problem,
    % \item \textbf{Special Symbols} (CHRL): Unnecessary punctuation are present in the text. For example: problem --\textgreater prob*lem
   % \item \textbf{Stop Words} (WRDL): Common stopwords such as the, is, at, which, and are present unnecessarily. For example: He fought fiercely.  --\textgreater He is fought fiercely.
    %\item \textbf{Whitespaces} (CHRL): Unnecessary spaces between words or characters. For example: Wedding --\textgreater We  dding
   % \item \textbf{Emojis} (WRDL): Presence of emoji's - extremely common in social media. For example: I am very happy today. --\textgreater I am very :-D today.
    %\item \textbf{Homoglyphs} (WRDL): Homoglyphs are characters, or glyphs with identical shapes. Again, very common in social media. For example: This is Neat --\textgreater This is N3at, WOW! --\textgreater W0W!
%\end{enumerate} 



==> schemes.tex <==
\label{intro}
The most important decision in introducing corruptions is selecting the location of the change. Instead of leveraging the internals of the model or any domain-specific knowledge about the data to identify the right words to be corrupted, we choose a model and data agnostic approach for general applicability. This leaves us with only a few options in selecting the locations within the document to introduce corruptions. We describe these schemes and provide our motivation for considering them below. In the next section, we empirically evaluate if there is a particular scheme that outperforms the other in generating useful corruptions.
\linebreak
\linebreak
\textbf{Random Corruption}: 
The simplest method to introduce corruptions to a document is to add them randomly. Any word in the document is eligible for a potential corruption using any of the techniques listed above. This is motivated by the fact that, by nature, all words in a document should be equally likely to get corrupted. All words are equally likely to be misspelled, noise can be present at any location in the document and any word may be expressed differently and yet, the document may still convey the same meaning. Thus, our first scheme is to randomly select words to be corrupted from the input document.
\linebreak
\linebreak
\textbf{Targeted Corruption}: 
Our goal is to ultimately test classification models. Therefore, an alternate hypothesis is that although all words in a document are equally likely to get corrupted, the result of corruptions would certainly be different for different words. Since, not all words are given equal importance by a model, this implies that words that are more important, should strongly affect the model's prediction upon corruption.

Local Interpretable Model-Agnostic Explanations (LIME) (todo: cite lime) is a popular black-box method to produce explanations of model predictions. For text inputs, the method returns a list of words in the document, ranked in decreasing order of importance, that were responsible for a particular prediction by the chosen model. In other words, the rank of a word can be interpreted as the importance of the word according to the model for a given prediction. Hence, our alternate scheme for selecting corruption targets is to prefer the words in the order generated by LIME. At first, this may seem to be equivalent to generating adversarial examples for text, except our goal is not to fool the classifier, but to produce enough variations in the test data.

\subsection{Overview of the Algorithm}
Our approach is best described as a pipeline of operations (Figure FF). The existing test dataset and the model being evaluated are provided as input. The only data cleaning we apply is to remove all punctuation from the input documents, except sentence delimiters. We apply both random and targeted schemes (using LIME) and select the words for corruption with just one additional condition - Stopwords are not eligible for corruption. We argue that stopwords convey very little information in the overall meaning of the document. Further, most models tend to give very little importance to stopwords (explicitly or indirectly). Thus, in the Random Corruption scheme, we do not consider stop words for random selection. With Targeted Corruption, if LIME recommends a stopword as having high importance, we ignore the word and pick the next important word. Table X shows some examples of explanation words produced by LIME. As will be elaborated in the next section, to keep the comparison fair in our experiments, only the documents for which we were able to generate a targeted corruption are eligible for random corruption. Once, the corruption targets are determined, we apply the desired corruption technique and produce a corresponding corrupted test set.

% show examples of lime selecting words

==> synonyms.tex <==
\label{intro}
One of the simplest ways to corrupt a given text document is to replace important words in the document with their synonyms. Depending on the selected words and their synonyms, this can drastically increase or decrease the readability of the document. Additionally, it is almost guaranteed to preserve most of the document's overall meaning and thus it's class label. We generate a synonym set for a word using Wordnet and replace the word with a randomly selected synonym from this set. In our experiments, we only consider words classified as Nouns, Adjectives, Verbs and Adverbs for corruption via synonym replacement. 

==> typos.tex <==
\label{intro}
With the amount of user-generated text data being exchanged on social media and other online channels, it is almost guaranteed that any datasets derived from these sources will exhibit human tendencies to make spelling errors. We account for two types of spelling errors:
\begin{enumerate}
    \item Typographical error (often abbreviated to typo) or spelling error that occur due to slips of the hand or finger while typing on electronic devices.
    \item Other spelling errors may be due to incorrect usage of words. We consider the following types of spelling errors in our corruptions, which may occur at a Character level (CHRL) or Word level (WRDL).
\end{enumerate}

Table ~\ref{typos-table} list the different techniques employed for introducing spelling errors in text. 




%\begin{enumerate}
    %\item \textbf{Missing Characters} (CHRL): A character is unintentionally dropped from a word. For example: problem --\textgreater  prblem
    %\item \textbf{Keyboard Proximity} (CHRL): A character can often be mis-typed incorrectly with a neighbouring character on the keyboard (we consider only the 'QWERTY' keyboard layout). For example: problem --\textgreater problrm
    %\item \textbf{Adjacent Character Swap} (CHRL): Adjacent characters in a word are interchanged accidentally. For example: likely --\textgreater liekly
    %\item \textbf{Character Repetition} (CHRL): A character is unintentionally pressed more than once. For example: problem --\textgreater pproblem.
    %\item \textbf{Case Change} (CHRL): The case of a character is changed due to accidentally holding on to the 'shift' key with a character key. For example: Wedding --\textgreater WEdding
    %\item \textbf{Homophones} (WRDL): Incorrect usage of words having the same pronunciation but different meanings, origins, or spelling. This type of typo is most likely to happen when we convert voice to text. For example: their --\textgreater there or brake --\textgreater break)
%\end{enumerate}
